Locally Adaptive Label Smoothing for Predictive Churn

Training modern neural networks is an inherently noisy process that can lead to high \emph{prediction churn} -- disagreements between re-trainings of the same model due to factors such as randomization in the parameter initialization and mini-batches -- even when the trained models all attain similar accuracies. Such prediction churn can be very undesirable in practice. In this paper, we present several baselines for reducing churn and show that training on soft labels obtained by adaptively smoothing each example's label based on the example's neighboring labels often outperforms the baselines on churn while improving accuracy on a variety of benchmark classification tasks and model architectures.

==> celeba_results.tex <==
\begin{table*}[H]
\small
\begin{tabular}{l|l|l|l|l|l}
\hline
Dataset               & Method                                          & Accuracy \%  & Churn \%     & Chrn Correct & Chrn Incorrect \\ \hline
                      & $k$-NN LS (k=100, b=0.1, a=0.9) & {\bf 90.02} (0.11) & {\bf 5.46} (0.32)  & {\bf 2.97} (0.18)      & 27.71 (1.74)       \\
                      & Label Smoothing (0.05)                             & 89.39 (0.29) & 6.77 (0.41)  & 3.81 (0.26)      & 31.67 (2.34)       \\
                      & Anchor (0.8)                                    & 89.87 (0.14) & 5.57 (0.28)  & 3.07 (0.21)      & 27.66 (1.38)       \\
CelebA        & L2 reg (0.01)                                   & 89.35 (0.16) & 6.85 (0.34)  & 3.92 (0.27)      & 31.62 (1.21)       \\
  Smiling       & L1 reg (0.5)                                    & 89.39 (0.26) & 6.71 (0.26)  & 3.61 (0.22)      & 32.48 (1.35)       \\
                      & Co-distill (CE, 0.5, 1000 warmup)                & 89.59 (0.29) & 6.31 (0.23)  & 3.66 (0.3)       & 29.47 (1.47)       \\
                      & Co-distill (KL, 0.5, 2000 warmup)                & 89.57 (0.22) & 6.1 (0.23)   & 3.34 (0.26)      & 29.66 (1.47)       \\
                      & Bitempered ($t_1$=0.9, $t_2$=2., n\_iters=5)       & 89.88 (0.18) & 6.44 (0.31)  & 3.56 (0.19)      & 31.96 (1.96)       \\
                      & Control                                         & 89.67 (0.19) & 7.3 (0.45)   & 4.06 (0.27)      & 35.34 (2.35)       \\ \hline
                      & $k$-NN LS (k=100, b=0.1, a=0.9) & {\bf 84.48} (0.21) & {\bf 7.7} (0.29)   & {\bf 4.64} (0.27)      & 24.44 (0.98)       \\
                      & Label Smoothing (0.005)                            & 83.73 (0.17) & 8.68 (0.46)  & 5.2 (0.35)       & 26.61 (1.28)       \\
                      & Anchor (0.9)                                    & {\bf 84.48} (0.2)  & 7.97 (0.39)  & 4.77 (0.22)      & 25.44 (1.58)       \\
CelebA  & L2 reg (0.001)                                  & 83.6 (0.14)  & 9.06 (0.32)  & 5.41 (0.24)      & 27.66 (1.03)       \\
     High                  & L1 reg (0.01)                                   & 83.59 (0.26) & 8.43 (0.23)  & 4.93 (0.23)      & 26.14 (1.16)       \\
     Cheekbone                 & Co-distill (CE, 0.5, 1000 warmup)                & 84.08 (0.21) & 8.96 (0.37)  & 5.33 (0.36)      & 28.11 (0.88)       \\
                      & Co-distill (KL, 0.5, 1000 warmup)                & 84.31 (0.08) & 8.57 (0.16)  & 5.06 (0.13)      & 27.39 (0.47)       \\
                      & Bitempered ($t_1$=0.5, $t_2$=4, n\_iters=5)       & 83.92 (0.13) & 7.84 (0.32)  & 4.75 (0.21)      & 24.01 (1)          \\
                      & Control                                         & 83.93 (0.56) & 10.18 (0.93) & 6.2 (0.89)       & 31.1 (2.22)        \\ \hline
                      & $k$-NN LS (k=500, a=0.8, b=0.9) & {\bf 96.69} (0.09) & {\bf 1.04} (0.21)  & {\bf 0.54} (0.14)      & 15.81 (3.52)       \\
                      & Label Smoothing (0.8)                              & 96.63 (0.09) & 1.26 (0.26)  & 0.64 (0.17)      & 18.8 (3.42)        \\
                      & Anchor (0.9)                                    & 96.02 (0.25) & 2.33 (0.25)  & 1.08 (0.15)      & 31.58 (5.11)       \\
 Phishing          & L2 reg (0.5)                                    & 96.51 (0.12) & 1.35 (0.3)   & 0.7 (0.21)       & 19.37 (4)          \\
                      & L1 reg (0.5)                                    & 95.38 (0.18) & 1.48 (0.34)  & 0.83 (0.24)      & 14.95 (4.08)       \\
                      & Co-distill (CE, 0.2, 2000 warmup)                & 96.02 (0.19) & 1.45 (0.26)  & 0.83 (0.21)      & 16.72 (4.13)       \\
                      & Co-distill (KL, 0.001, 1000 warmup)              & 95.94 (0.33) & 1.51 (0.2)   & 0.65 (0.18)      & 20.95 (6.14)       \\
                      & Bitempered ($t_1$=0.9, $t_2$=1.0)                     & 96.26 (0.37) & 2.32 (0.69)  & 1.23 (0.53)      & 30.19 (8.51)       \\
                      & Control                                         & 96.3 (0.32)  & 2.25 (0.59)  & 1.21 (0.38)      & 29.05 (7.93)       \\ \hline
\end{tabular}
\caption{Results for the CelebA and Phishing datasets.}% We observe that our $k$-NN label smoothing consistently matches or outperforms baselines, improving \emph{both} churn and accuracy.}
\label{table:celeba}
\end{table*}



==> svhn_results.tex <==
\begin{table*}[H]
\small
\begin{tabular}{l|l|l|l|l|l}
\hline
Dataset       & Method                                                                    & Accuracy \% & Churn \% & Chrn Correct & Chrn Incorrect  \\ \hline
              & \begin{tabular}[c]{@{}l@{}}k-NN LS (a=1, b=0.9,k=10)\end{tabular} & {\bf 88.98} (0.33)      & {\bf 10.98} (0.28)   & {\bf 4.64} (0.29)            & 62.23 (1.22)             \\
              & Label Smoothing ($a$=0.9)                                                      & 87.26 (0.73)      & 13.46 (0.62)   & 5.31 (0.57)            & 67.2 (1.44)              \\
              & Anchor (a=\todo{fill here and below})                                                 & 87.17 (0.16)      & 12.48 (0.39)   & 5.19 (0.2)             & 61.66 (1.85)             \\
SVHN          & L2 reg (0.5)                                                          & 88.16 (0.35)      & 11.85 (0.35)   & 5.07 (0.16)            & 62.73 (2.1)              \\
              & L1 reg (0.2)                                                          & 74.18 (3.41)      & 22.89 (3.74)   & 9.58 (4.04)            & 59.36 (5.7)              \\
              & codistill (CE, 0.5)                                                       & 87.64 (0.64)      & 12.46 (0.48)   & 5.16 (0.51)            & 63.82 (1.67)             \\
              & codistill (KL, 0.5)                                                       & 87.52 (0.45)      & 13.01 (0.3)    & 5.54 (0.33)            & 65.44 (1.46)             \\
              & Bitempered ($t_1$=0.5, $t_2$=1., n\_iters=5)                                  & 88.04 (0.5)       & 12.03 (0.3)    & 5.26 (0.3)             & 62.48 (1.83)             \\
              & Control                                                                   & 86.64 (0.54)      & 14.64 (0.51)   & 6.03 (0.5)             & 69.59 (1.32)             \\ \hline
              & $k$-NN LS (k=5, a=0.9, b=0.9)                             & {\bf 98.23} (0.11)      & {\bf 1.52} (0.12)    & {\bf 0.7} (0.1)              & 47.16 (3.39)             \\
              & Label Smoothing (0.9)                                                        & 98.15 (0.07)      & 1.65 (0.05)    & 0.71 (0.07)            & 50.73 (2.62)             \\
              & Anchor (1.0)                                                              & 97.72 (0.11)      & 2.66 (0.2)     & 1.21 (0.14)            & 64.51 (4.13)             \\
MNIST         & L2 reg (0.5)                                                              & 98.08 (0.1)       & 1.67 (0.12)    & 0.8 (0.08)             & 46.65 (3.2)              \\
              & L1 reg (0.01)                                                             & 97.67 (0.29)      & 2.51 (0.31)    & 1.3 (0.27)             & 56.8 (2.84)              \\
              & Co-distill (CE, 0.2, 2000 warmup)                                          & 98.08 (0.06)      & 2.08 (0.11)    & 0.98 (0.07)            & 58.6 (3.91)              \\
              & Co-distill (KL, 0.05, 1000 warmup)                                         & 97.98 (0.14)      & 2.16 (0.16)    & 0.97 (0.13)            & 59.56 (3.64)             \\
              & Bitempered ($t_1$=0.9, $t_2$=1.0, n\_iters=5)                                 & 98.09 (0.2)       & 2.04 (0.15)    & 1.07 (0.14)            & 55.82 (4.32)             \\
              & Control                                                                   & 97.98 (0.13)      & 2.28 (0.13)    & 0.96 (0.07)            & 63.36 (2.55)             \\ \hline
              & $k$-NN LS (k=10, a=1, b=0.5)                              & 88.89 (0.14)      & {\bf 6.94} (0.18)    & {\bf 3.27} (0.15)            & 36.26 (1.09)             \\
              & Label Smoothing (0.8)                                                        & 88.46 (0.17)      & 7.2 (0.46)     & 3.32 (0.28)            & 36.63 (2.02)             \\
              & Anchor                                                                    & 88.55 (0.14)      & 7.53 (0.45)    & 3.6 (0.23)             & 37.78 (2.29)             \\
Fashion  & L2 reg (0.5)                                                               & 88.52 (0.19)      & 7.86 (0.36)    & 3.59 (0.18)            & 40.38 (1.81)             \\
    MNIST          & L1 reg (0.1)                                                              & 86.88 (0.35)      & 8.24 (0.55)    & 3.88 (0.41)            & 36.81 (2.63)             \\
              & Co-distill (CE, 0.5, 2000 warmup)                                          & 88.76 (0.21)      & 7.51 (0.39)    & 3.67 (0.3)             & 37.98 (1.71)             \\
              & Co-distill (KL, 0.5, 2000 warmup)                                          & 88.85 (0.35)      & 7.83 (0.43)    & 3.68 (0.29)            & 40.59 (2.4)              \\
              & Bitempered ($t_1$=0.7, $t_2$=2)                                                 & 88.7 (0.29)       & 7.36 (0.47)    & 3.5 (0.19)             & 37.24 (3.04)             \\
              & Control                                                                   & {\bf 88.95} (0.26)      & 9.13 (0.51)    & 4.42 (0.4)             & 46.99 (2.49)             \\ \hline
\end{tabular}
\caption{Results for SVHN, MNIST, and Fashion MNIST datasets.}
\label{table:svhn}
\end{table*}
